DetailGen3D: Generative 3D Geometry Enhancement via Data-Dependent Flow

Modern 3D generation methods can rapidly create shapes from sparse or single views, but their outputs often lack geometric detail due to computational constraints. We present DetailGen3D, a generative approach specifically designed to enhance these generated 3D shapes. Our key insight is to model the coarse-to-fine transformation directly through data-dependent flows in latent space, avoiding the computational overhead of large-scale 3D generative models. We introduce a token matching strategy that ensures accurate spatial correspondence during refinement, enabling local detail synthesis while preserving global structure. By carefully designing our training data to match the characteristics of synthesized coarse shapes, our method can effectively enhance shapes produced by various 3D generation and reconstruction approaches, from single-view to sparse multi-view inputs. Extensive experiments demonstrate that DetailGen3D achieves high-fidelity geometric detail synthesis while maintaining efficiency in training.

==> sec/2.5_preliminaries.tex <==
\section{Preliminaries}
\label{sec:method}

\setlength{\parindent}{2em}

\emph{DetailGen3D} adopt Vecset as our 3D representation, proposed in 3DShape2Vecset~\cite{zhang20233dshape2vecset3dshaperepresentation}, which uses a 3D-VAE to transform 3D model into Vecset form. To obtain a 3D model's corresponding Vecset, 3DShape2Vecset firstly sample point cloud $X$ from surface then downsample it randomly, denoted as query points $X_0$. Lastly, the cross attention is applied to $X$ and $X_0$ to obtain Vecset. The 3D-VAE's decoder, composed several self attention layers and a cross attention layer, transform Vecset to occupancy field with given query, i.e., 3D points in space. 

